Local Differential Privacy for Physical Sensor Data and Sparse Recovery

In this work we explore the utility of locally differentially private thermal sensor data. We design a locally differentially private recovery algorithm for the 1-dimensional, discrete heat source location problem and analyse its performance in terms of the Earth Mover Distance error. Our work indicates that it is possible to produce locally private sensor measurements that both keep the exact locations of the heat sources private and permit recovery of the "general geographic vicinity" of the sources. We also discuss the relationship between the property of an inverse problem being ill-conditioned and the amount of noise needed to maintain privacy.

==> experiments.tex <==
%!TEX root = ./main.tex

\subsection{Experimental Results}

In this section we present experimental results. The source vectors are $n$ dimensional vectors where the possible source locations are $\{\frac{1}{n}, \cdots, 1\}$. The sensors are placed at locations $\{\frac{1}{m}, \cdots, 1\}$. The diffusion constant, $\mu$, is equal to $1/2$ for all experiments. In all graphs, all but one of the variables $n$, $m$, $t$, $\sigma$, $\epsilon$ or $\delta$ are kept constant. The EMD between two vectors is computed by first scaling both vectors to have unit $\ell_1$ norm, then computing the EMD between the normalised vectors. In experiments where $k=1$, the source is always at 0.5. If $k>1$ then $k$ source locations are chosen uniformly at random. All sources have unit intensity. 

All code was run in MATLAB R2016a. In all cases where confidence bars are present, the bars are 95\% confidence intervals computed after performing 10 trials with fixed parameters. The sensitivity $\triangle_2(A)=\max_i\|A_i-A_{i+1}\|_2$ was computed exactly for each trial.

Figure \ref{nonprivateemderror} shows the results of simulations of Algorithm \ref{l1mini} on noisy thermal measurements. These simulations suggest that Theorem \ref{main} is asymptotically tight in $n$ and $\sigma$. It is more difficult to determine whether the empirical results suggest tightness is $T$, although it certainly does not contradict it. The result for $m$ is inconclusive, our upper bound of $O(1)$ and lower bound of $O(1/\sqrt{m})$ differ by a factor of $\sqrt{m}$. The simulations suggest that the true error rate behaves something like $1+\frac{1}{\sqrt{m}}$ since the error decays but not all the way to 0. 

\begin{figure}
\centering
\begin{subfigure}{.24\textwidth}
	\centering
	\includegraphics[width=1\linewidth]{new_sigma_EMD}
	\caption{Dependence on $\sigma$}
	\label{fig:sub21}
\end{subfigure}\hspace{0.05in}%
\begin{subfigure}{.24\textwidth}
	\centering
	\includegraphics[width=1\linewidth]{m_EMD}
	\caption{Dependence on $m$}
	\label{noisym}
\end{subfigure}\hspace{0.05in}
\begin{subfigure}{.24\textwidth}
	\centering
	\includegraphics[width=1\linewidth]{t_EMD}
	\caption{Dependence on $t$}
	\label{tvariesEMD}
\end{subfigure}\hspace{0.05in}%
\begin{subfigure}{.24\textwidth}
	\centering
	\includegraphics[width=1\linewidth]{n_EMD}
	\caption{Dependence on $n$}
	\label{nvariesEMD}
\end{subfigure}%\hspace{0.2in}%
\caption{Empirical results for the EMD error of experiments running Algorithm $R$ on measurement data with added gaussian noise with variance $\sigma^2$. Unless specified otherwise, $n=100$, $m=50$, $T=0.5$, $\sigma=0.1$ and $k=1$. In \eqref{tvariesEMD}, $\sigma=0.2$. In \eqref{nvariesEMD}, $T=0.05$ and $\sigma = 0.2$.}
\label{nonprivateemderror}
%\vspace{-0.1in}
\end{figure}

Figure \ref{privateemderror} (in Appendix \ref{furtherexperiments}) shows the results of simulations of our locally differentially private recovery algorithm. The results suggest that Theorem \ref{privatemain} is asymptotically tight in $n$ and $m$. It is difficult to determine the asymptotic nature in $T$ from the empirical result however the shape is consistent with the upper bound given. In particular both empirical and theoretical results imply that the EMD error increases both as $T\to 0$ and $T\to\infty$.
